Cosmic Whispers of the Early Universe: Gravitational Waves and Dark Matter from Primordial Black Holes

Various mechanisms have been suggested for the formation of Primordial Black Holes (PBHs), and this thesis focuses on the standard mechanism based on the critical collapse of cosmological fluctuations. The underlying idea is that during inflation, a period of rapid expansion in the early Universe, large cosmological fluctuations could have been generated. After inflation, when the cosmic horizon reached a size comparable to these fluctuations, if the latter were high enough, they could collapse and form a PBH. Beyond the fascinating possibility that these compact objects might make up all or part of the Dark Matter (DM) we observe today, their formation and existence is also associated with the generation of gravitational waves (GWs). These waves could contribute to the merger events observed by the LIGO/Virgo/KAGRA Collaboration (LVK) or account for signals detected by pulsar timing array experiments (PTA). In the first part of this thesis, we investigate the PBH scenario, examining the computation of the abundance beyond the Gaussian paradigm. In the second part, we discuss how PBH formation can produce a stochastic GW background and how observations, related to recent experiments such as LVK and PTA collaborations, can help in distinguishing between different PBH production models. Finally, in the last part, we investigate some aspects of the interplay between black holes and fundamental physics in the early Universe, describing some characteristics and challenges of various PBH production models.

==> Include/Frontmatter/Titlepage.tex <==
\begin{frontespizio}
% Remember: After editing this file, delete the cache and recompile
%---------------------Definizione font---------------------%
\Preambolo{\renewcommand{\fronttitlefont}{\fontsize{18}{18}\bfseries}}
%----------------------------------------------------------%
	% \frontinstitutionfont 	Neretto, 14/17 
	% \frontdivisionfont 		Tondo, 12/16 
	% \frontpretitlefont 		Maiuscoletto, 10/12
	% \fronttitlefont 		Neretto, 17/21 
	% \frontsubtitlefont 		Tondo, 12/14
	% \frontfixednamesfont 		Tondo, 12/14 
	% \frontnamesfont 		Neretto, 12/14 
	% \frontsmallfont 		Neretto, 9/11 
	% \frontfootfont	 	Neretto, 12/14 

	% \bfseries	Grassetto
	% \itshape	Corsivo
	% \scshape	Maiuscoletto
%----------------------------------------------------------%
\Margini{4cm}{3cm}{3cm}{3cm}				% Margini sinistro, in basso, destro e in alto
\Logo[4cm]{Figures/Logo/logo_sapienza_new.jpg}
%\Universita{Roma}
\Istituzione{Sapienza University of Rome}
%\Facolta{Civil and Industrial Engineering}		% = 'Facolta di Ingegneria Civile ed Industriale'
\Divisione{Department of Physics}		% = 'Facolta di Ingegneria Civile ed Industriale'
%\Dipartimento{Ingegneria Meccanica e Aerospaziale}	% = 'Dipartimento di Ingegneria Meccanica e Aerospaziale'
%\Corso[Master Degree]{Aeronautical Engineering}
\Scuola{PhD in THEORETICAL PHYSICS}
\Titoletto{Thesis For The Degree Of Doctor Of Philosophy}
\Titolo{Cosmic Whispers of the Early Universe:
\\Gravitational Waves and Dark Matter 
\\from Primordial Black Holes}
%\Sottotitolo{}
\Punteggiatura{}					% Modifica la punteggiatura dopo 'Candidato', 'Realatore' ecc. (vuoto per togliere)
\NCandidato{Candidate}					% Sostituisce 'Candidato' con '...'
\Preambolo{\renewcommand{\frontsmallfont}[1]{\small}}
\Candidato[1924537]{Antonio Junior Iovino}
%\Candidato{\small{1532252}}
\NRelatore{Thesis Advisor}{Relatori}			% Sostituisce 'Relatori' con 'Advisor' (permette anche di scrivere più relatori)
\Relatore{Prof. Alfredo Leonardo Urbano}
%\Correlatore{}
%\Rientro{1cm}						% Rientro di Relatore e Candidato
\Piede{Academic Year MMXXIII-MMXXIV (XXXVII cycle)}					% A fondo pagina
\end{frontespizio}
\IfFileExists{\jobname-frn.pdf}{}{%
\immediate\write18{pdflatex \jobname-frn}}
